Detecting Affective Flow States of Knowledge Workers Using Physiological Sensors

Flow-like experiences at work are important for productivity and worker well-being. However, it is difficult to objectively detect when workers are experiencing flow in their work. In this paper, we investigate how to predict a worker's focus state based on physiological signals. We conducted a lab study to collect physiological data from knowledge workers experienced different levels of flow while performing work tasks. We used the nine characteristics of flow to design tasks that would induce different focus states. A manipulation check using the Flow Short Scale verified that participants experienced three distinct flow states, one overly challenging non-flow state, and two types of flow states, balanced flow, and automatic flow. We built machine learning classifiers that can distinguish between non-flow and flow states with 0.889 average AUC and rest states from working states with 0.98 average AUC. The results show that physiological sensing can detect focused flow states of knowledge workers and can enable ways to for individuals and organizations to improve both productivity and worker satisfaction.

==> 55_Statistical_analysis_of_physiological_features.tex <==

\subsection{Statistical Analysis of Physiological Measures}
To better understand how to predict focus state based on physiological measures, we first perform statistical analyses to identify how different physiological measures are related to different focus states. In the following statistical analyses, we used JMP software (version 12) to perform statistical tests with each type of physiological data after data cleaning (described in section \ref{Methodology}). Physiological readings recorded from each study task are grouped by the corresponding labels balanced flow, automatic flow, or not-flow. For example, heart rate data (bpm) recorded during from participant 2 during the Research Task was aggregated and the mean of samples during that task, resulting in an average heart rate for p2 during the Research Task. The procedure was repeated for each physiological data type, for each participant, and across all three tasks. 

For each physiological data type, we conducted a repeated measures one-way ANOVA with the participant as a random factor and the focus state label as a fixed factor (3 levels for not-flow, automatic flow, and balanced flow). When the data violated ANOVA's requirement for sphericity according to Mauchly's Test, the Huynh-Feldt correction \cite{huynh1978some} was applied to adjust the degrees of freedom in the F-test for a more conservative estimate. When data violated ANOVA's requirement for normality (i.e., significant result in the Shapiro-Wilk W Test), the non-parametric Friedman's test (reported with the Chi-squared statistic, $X^2$) and the Wilcoxon signed rank test for post-hoc comparisons was used instead of a parametric ANOVA and contrasts. For multiple comparisons, such as when comparing pairwise contrasts among the three labels, the Bonferroni-Holm Correction \cite{holm1979simple} was applied to adjust the alpha level for a conservative estimate. For the sake of brevity, we report only the statistically significant relationships. 

\subsubsection{Heart Rate Variability}
Heart rate and heart rate variability are traditionally used as measures of arousal and balance in sympathetic/parasympathetic activity. The average heart rates during the tasks were not significantly different. However, some measures of heart rate variability were different across the tasks, specifically, time-domain measures of rmssd and sdNN, frequency-domain measures of LF and total\_power, and non-linear measures of SD2 and SD1/SD2. rmssd was significantly higher in the not-flow condition (mean=101.3ms, sd=40.8) than in the other two conditions (mean=73.1ms, sd=27.2 for balanced flow and mean=71.3, sd=30.2ms for automatic flow), F[1.4,15.6]=6.18, p=0.017. Similarly, sdNN was higher in the not-flow condition (mean=137.6, sd=85.4) than in the other two conditions (mean=94.5ms, sd=59.6 for balanced flow and mean=80.0ms, sd=51.1 for automatic flow), $X^2$(2)=0.5, p=0.009. %Typically, rmssd and sdNN are used as measures of variability in the beat-to-beat intervals. Prior literature has associated higher variability with parasympathetic nervous activity to less perceived mental stress \cite{orsila2008perceived} and lower cognitive demand (i.e., perceptual difficulty and sustained attention) \cite{luque2016heart}. 
Additional data from the frequency domain features of HRV are also consistent, total\_power in the not-flow condition (mean=14330, sd=16048) being higher than in the other two conditions (mean=6665, sd=11210 for balanced flow and mean=5579, sd=8933 for automatic flow), $X^2$(2)=15.2, p<0.001. %Total\_power can be roughly interpreted as a measurement of variation of the heart rate. Thus, it is surprising that the Patent task, which was designed to be the most demanding, would be associated with time-domain features of HRV commonly related to low stress. 

Another frequency domain feature, LF (low-frequency), has been attributed to sympathetic cardiac tone but more recently and specifically to the baroreflex (blood pressure) function \cite{goldstein2011low}, and is consistently higher in the not-flow condition (mean=5050, sd=4991) compared with the other two conditions (mean=2658, sd=4894 for balanced flow and mean=2146, sd=3870 for automatic flow), $X^2$(2)=14, p<0.001. %In contrast to other HRV features, a higher low-frequency feature of HRV points indicates an expected increased level of perceived stress in the Patent task.

\subsubsection{Pupil Diameter}
Pupil size has been found in prior studies to be correlated with cognitive load and higher perceived stress \cite{bailey2008understanding}. We found that mean pupil diameter was significantly smaller (less dilated) in the not-flow condition (mean=2.66mm, sd=0.27mm) than in the other two tasks (mean=2.76mm, sd=0.28mm for balanced flow and mean=2.85mm, sd=0.32mm for automatic flow), F[2,22]=9.27, p=0.0012. After correcting for multiple comparison, the contrast between the balanced flow and automatic flow conditions was only at the p=0.065 significance level, indicating a much stronger difference between the not-flow and automatic flow conditions in terms of pupil diameter. %Typically, it has been found that pupil size increases with the difficulty of the task, so it is surprising that we found the smallest pupil size in our most difficult task.

\subsubsection{Skin Conductance}
Skin conductance was measured on the non-dominant wrist with the MS Band 2. We found that the rmssd of skin conductance data in the automatic flow condition (mean=0.004$\mu$S, sd=0.002$\mu$S) was significantly lower than in the other two conditions (mean=0.020$\mu$S, sd=0.017$\mu$S for balanced flow and mean=0.013$\mu$S, sd=0.012$\mu$S for not-flow), $X^2$(2)=9.5, p=0.0087. Even though we did not find any significant differences in the mean or median of the skin conductance levels across the conditions, our data shows that skin conductance varied quite a bit less in the automatic flow condition than the other conditions. 

Another measure derived from the skin conductance data is the phasic signal, characterized by the peaks in the signal attributed to an electro-dermal response, typically attributed to moments of arousal. The number of peaks in a given period is a discrete number, and to control for slight variations in time length of the recorded data, we divided the peak count by the number of skin conductance samples in 1 second (which in our case was 8 because our skin conductance data was sampled at 8Hz) to yield a derived measure of peaks per second. The results show that the balanced flow condition (mean=0.042 peaks/sec, sd=0.032) had a significantly higher peak rate than the automatic flow condition (mean=0.015 peaks/sec, sd=0.025), $X^2$(2)=11.17, p=0.0038. The not-flow condition also had a higher rate (mean=0.023 peaks/sec, sd=0.022) than the automatic flow condition, but after Bonferroni-Holm Correction, the post-hoc Wilcoxon signed rank test was not significant, $X^2$(2)=1.61, p=0.10. %Peaks typically correspond to moments of arousal, and thus it is not surprising that the balanced flow-inducing Research task would be more stimulating than the less demanding Spreadsheet task.

\subsubsection{Physiological Features Associated with Focus States}
The statistical analysis revealed that some physiological parameters may be good for discriminating certain focus states from others. In summary, the data suggest that the not-flow condition (that is, a state that overly challenging, rating lowly across flow characteristics) seems to be distinguished by less pupil dilation, higher rmssd, sdNN, LF, and total\_power for HRV. The overly easy, automatic flow condition is distinguished by a lower rmssd in skin conductance levels. The balanced-flow inducing balanced flow condition is most distinguished by a greater number of electro-dermal response peaks. The results of this statistical analysis can help inform which features might have greater discriminative power when building a machine learning model to predict a user's focus state based on physiology. 

\subsubsection{Quantifying Physiological Correlates of Rest State}
The previous analyses have looked at a 3-way comparison between the 3 conditions. In this section, we describe a 4-way comparison that includes the 3 conditions and a fourth state, rest. For each participant, we grouped together the data collected from the three rest periods following each task where participants sat quietly looking at a slideshow of nature photos. We followed the same statistical analysis methods as described above, adjusting as necessary for assumptions of ANOVA. The results show that physiological responses (pupil diameter and HRV) measured during rest did have some significant differences from when participants were engaged in the tasks. 

Mean pupil diameter was significantly larger during rest (mean=3.08mm, sd=0.42mm) than when performing a task (mean=2.85mm, sd=0.32mm for automatic flow, mean=2.76mm, sd=0.28mm for balanced flow, and mean=2.66mm, sd=0.27mm for not-flow), F[3,33]=25.04, p<0.001. Similarly, the data revealed that the variance in pupil diameter was much larger during rest (mean=0.089, sd=0.046) than during a task (mean=0.023, sd=0.012 for automatic flow, mean=0.021, sd=0.010 for balanced flow, and mean=0.020, sd=.012mm for not-flow), $X^2$(3)=21.9, p<0.0001.

For HRV, the frequency domain metrics of the LF/HF ratio and LFnu both showed a strong difference between rest and when performing a task. The LF/HF ratio during rest was significantly higher (mean=1.54, sd=0.37) than during each of the tasks (mean=1.23, sd=0.73mm for not-flow, mean=0.86, sd=0.43 for automatic flow, mean=0.97, and sd=0.31 for balanced flow), $X^2$(3)=10.7, p=0.013. The normalized low frequency (LFnu) showed an identical pattern with rest being significantly higher than each of the tasks ($X^2$(3)=10.7, p=0.013). The time domain metrics of HRV also show some relationships, though they are not as dramatic as the LF/HF ratio. The sdNN during rest, similar to the not-flow condition, is significantly higher (mean=147.1ms, sd=79.7) than in the automatic flow (mean=80.0, sd=51.1) and balanced flow (mean=94.5, sd=59.6) conditions, $X^2$(3)=14.5, p<0.0023. The rmssd metric, however, shows that the not-flow condition (mean=101.3, sd=40.8) is higher than the other conditions including during rest (mean=75.3, sd=24.0), F[3,33]=5.19, p=0.005.

In summary, idle states where the participant was simply viewing nature photos silently were correlated with significantly greater mean and variance of pupil dilation as well as a higher LF/HF and LFnu HRV, both typically associated with sympathetic activity. In contrast, the higher sdNN and moderate rmssd during rest suggests more parasympathetic activity associated with more restful states.

==> 65_Discussion_statistical_analysis.tex <==
\subsection{Physiological Correlates of Flow States in Work Tasks}
In this section, we address research question 2 and discuss how flow and non-flow states are correlated with physiological measures. The results of the statistical analysis show that the balanced flow state is most distinguished by high number of skin conductance peaks. Skin conductance is often associated as a measurement of arousal, with peaks often attributed to moments of insight or recognition. We found that skin conductance peaks were more common in interesting, arousing balanced flow states in which participants read and summarized an interesting paper. Our analysis also shows the automatic flow state is characterized by a lower rMSSD in skin conductance levels than the other states, consistent with the expectation that changes in arousal in uninteresting overly easy tasks to be low.

%The statistical analysis of which physiological parameters are correlated with flow and non flow states revealed some interesting patterns that seem to paint a different picture of flow than prior research. In particular, measures of pupil diameter seem to be negatively correlated with cognitive load, with the highest in the more relaxed conditions (Rest) and lowest in conditions requiring high cognitive load (Patent Task), the opposite of what has been found in previous research where pupil diameter is positively correlated with cognitive load. Given the validity of our self-reported manipulation check of the difficulty of tasks, we speculate that photographic images of nature scenes might induce a larger pupil size because the participant has to defocus somewhat to see the entire image rather than reading text in the other tasks. Perhaps the subtle difference in luminance of the photographs compared with the typical white background found in other tasks might have contributed to the difference in pupil size. 
% If we exclude pupil features from the rest vs not-rest classifier, accuracy averaged across participants drops to 72\% (sd=17\%), with precision at 73\% and recall at 75\%, which can still be potentially useful.

Measures of heart rate variability also had a different relationship with cognitive load and stress than expected. Higher HRV is typically associated with relaxed states and the activation of the parasympathetic activity in the autonomic nervous system. Interestingly, HRV (rMSSD, sdNN, total\_power) was significantly higher in the most challenging task (Patent) than the other task. This finding can be interpreted in a couple of ways. The first interpretation is that participants were the most calm and relaxed during the Patent task, even though it was self-reported as being the most challenging and least enjoyable task. They might have given up on the task because it was so hard and stopped trying and equilibrated to a relaxed, disengaged state. However, this interpretation does not match with our manipulation check on the difficulty level of the tasks and also is not what our participants reported, as they all said they tried to read the material and process it throughout the task. Another interpretation of the association of high HRV with challenge task is similar to the study of expert pianists who were told to play a piece they never played before \cite{ullen201010}. In that study, the more experienced pianists actually had higher HRV values when they played a challenging, new piece, and the authors reasoned that the expert pianists were able recruit parasympthetic nervous system to moderate their (hyper-)arousal to deal with the novel challenge. Qualitative feedback from participants showed that all participants found the task challenging, exceeding their abilities to comprehend complex legal jargon in an unfamiliar technical domain, but many reported that they saw it as a challenge to learn about something new and to develop a skill (reading patent specifications). This reframing of a challenging task might be part of a self-soothing parasympthetic strategy by our expert researcher participants who regularly encounter new challenges in their daily work. 
